The Impact of Gait Pattern Personalization on the Perception of Rigid Robotic Guidance: A Pilot User Experience Evaluation

Exoskeletons modulate human movement across diverse applications, from performance augmentation to daily-life assistance. These systems often enforce specific kinematic patterns to mitigate injury risks and motivate users to keep moving despite diminished capacity. However, little is known about users' perception of such robot-imposed guidance, especially when personalized to the uniqueness of individual human walk. Given the usually substantial computational cost for personalization, understanding its subjective impact is essential to justify its implementation over standard patterns. Ten unimpaired participants completed a within-subject experiment in a multi-planar treadmill-based exoskeleton that enforced three different gait patterns: personalized, standard, and a randomly selected pattern from a publicly available database. Personalization was achieved using a data-driven framework that predicts hip, knee, and pelvis trajectories from walking speed, anthropometric, and demographic data. The standard pattern was obtained by averaging gait patterns from the aforementioned database. After each condition, participants rated enjoyment, comfort, and perceived naturalness. Knee joint interaction forces were also recorded. Subjective ratings revealed no significant differences among patterns, despite all trajectories being executed with high accuracy. However, gait patterns experienced last were rated as significantly more comfortable and natural, indicating adaptation to the system. Higher interaction forces were observed only for the random vs. standard pattern. Personalizing gait kinematics had minimal short-term influence on user experience relative to the dominant effect of adaptation to the exoskeleton. These findings highlight the importance of integrating subjective feedback and accounting for user adaptation when designing personalized robot controllers.

==> KinematicModel.tex <==
\color{blue}

\subsection{Kinematic loop-closure formulation}

The hip module forms a closed kinematic chain that can be expressed by closing two branches of the loop, either at the hip joint $H$ or at the upper hinge $E$ of the parallel mechanism (see Fig.~\ref{fig:kinematic_model}). In the following, we derive the homogeneous positions of $H$ and $E$ from both perspectives.

\subsubsection{Top branch (pelvis $\rightarrow H \rightarrow M \rightarrow E$)}
The pelvis plate pose is defined by the measured rotations $\alpha,\beta,\gamma$:
\begin{equation}
R^\mathcal{F}_\mathcal{P} = R_x(\alpha)R_y(\beta)R_z(\gamma), \qquad
T^\mathcal{O}_\mathcal{P} = T^\mathcal{O}_\mathcal{F} + T^\mathcal{F}_\mathcal{P} .
\end{equation}
The hip joint is located at a calibrated offset $T^\mathcal{P}_\mathcal{H}$:
\begin{equation}
T^\mathcal{O}_\mathcal{H}\big|_{\text{top}} = T^\mathcal{O}_\mathcal{P} + R^\mathcal{F}_\mathcal{P} T^\mathcal{P}_\mathcal{H} .
\end{equation}
The hip orientation in $O$ is given by
\begin{equation}
R^\mathcal{O}_\mathcal{H} = R^\mathcal{F}_\mathcal{P} R^\mathcal{P}_\mathcal{H}, \qquad
R^\mathcal{P}_\mathcal{H} = R_x(\theta_{fl})R_y(\theta_{ab})R_z(\theta_{ro}) .
\end{equation}
Propagating along the thigh yields
\begin{equation}
T^\mathcal{O}_\mathcal{E}\big|_{\text{top}} = T^\mathcal{O}_\mathcal{H}\big|_{\text{top}} + R^\mathcal{O}_\mathcal{H}
\begin{bmatrix}
0 \\ -l_n \\ -l_m
\end{bmatrix}.
\end{equation}

\subsubsection{Bottom branch (actuator plane $\rightarrow E \rightarrow B \rightarrow H$)}
The actuator plane $A$ is rotated by $\theta_A$ about the $x$-axis:
\begin{equation}
R^\mathcal{O}_\mathcal{A} = R_x(\theta_A).
\end{equation}
The distal ends of the linear actuators are
\begin{equation}
T^\mathcal{A}_{P_{\mathrm{ext}}} =
\begin{bmatrix}
\frac{l_c}{2} \\ p_{\mathrm{ext}} + d \\ 0
\end{bmatrix}, \quad
T^\mathcal{A}_{P_{\mathrm{int}}} =
\begin{bmatrix}
-\frac{l_c}{2} \\ p_{\mathrm{int}} + d \\ 0
\end{bmatrix}.
\end{equation}
With link orientations $R^\mathcal{A}_{P_{\mathrm{ext}}E} = R_z(\theta_1)$ and $R^\mathcal{A}_{P_{\mathrm{int}}E} = R_z(-\theta_2)$, the hinge $E$ satisfies
\begin{equation}
T^\mathcal{A}_\mathcal{E} = T^\mathcal{A}_{P_{\mathrm{ext}}} + R^\mathcal{A}_{P_{\mathrm{ext}}E}
\begin{bmatrix}0\\l_1\\0\end{bmatrix}
= T^\mathcal{A}_{P_{\mathrm{int}}} + R^\mathcal{A}_{P_{\mathrm{int}}E}
\begin{bmatrix}0\\l_2\\0\end{bmatrix}.
\end{equation}
In world coordinates:
\begin{equation}
T^\mathcal{O}_E\big|_{\text{bot}} = R^\mathcal{O}_\mathcal{A} T^\mathcal{A}_\mathcal{E} .
\end{equation}
Propagating further:
\begin{align}
T^\mathcal{O}_\mathcal{B} &= T^\mathcal{O}_\mathcal{E}\big|_{\text{bot}} + R^\mathcal{O}_\mathcal{A} R_x(\theta_E)
\begin{bmatrix}0\\ l_n \\ 0\end{bmatrix}, \\
T^\mathcal{O}_\mathcal{H}\big|_{\text{bot}} &= T^\mathcal{O}_\mathcal{B} + R^\mathcal{O}_\mathcal{A} R_y(\theta_B)
\begin{bmatrix}0\\ 0\\ l_m\end{bmatrix}.
\end{align}

\subsubsection{Loop-closure conditions}
The kinematic loop can then be closed either at the hip or at the hinge:
\begin{align}
&\text{Closure at $H$:} & T^\mathcal{O}_\mathcal{H}\big|_{\text{top}} &= T^\mathcal{O}_\mathcal{H}\big|_{\text{bot}} , \\
&\text{Closure at $E$:} & T^\mathcal{O}_\mathcal{E}\big|_{\text{top}} &= T^\mathcal{O}_\mathcal{E}\big|_{\text{bot}} .
\end{align}
The first is convenient for forward kinematics (joint $\rightarrow$ actuator space), while the second is more natural for inverse kinematics (actuator $\rightarrow$ joint space).

\color{black}

\subsubsection*{\textbf{Pelvis plate}}

The spherical hip joint of the exoskeleton, denoted as \(H\) in Fig.~\ref{Fig:2}.a, is rigidly mounted on the pelvis plate. Since its position must be adaptable to accommodate different user sizes, a translation \(\mathbf{T}_\mathcal{H}^\mathcal{P}\) from the pelvis plate origin \(P\) to the hip joint \(H\) is included in the model.
The position of \(H\) with respect to the world frame \(\mathcal{O}\) is computed as:
\begin{equation} \label{eq:1}
\mathbf{T}_\mathcal{H}^\mathcal{O} = \mathbf{T}_\mathcal{P}^\mathcal{O} + \mathbf{R}_\mathcal{F}^\mathcal{O}\mathbf{R}_\mathcal{P}^\mathcal{F} \mathbf{T}_\mathcal{H}^\mathcal{P}.
\end{equation}
%\begin{itemize}
    %\item 
Here, the orientation of frame \(\mathcal{F}\) coincides with that of the world frame \(\mathcal{O}\), so the rotation matrix \(\mathbf{R}_\mathcal{F}^\mathcal{O}\) is the identity matrix. \(\mathbf{R}_\mathcal{P}^\mathcal{F}\) is the pelvis plate’s orientation relative to the fixed frame \(\mathcal{F}\), obtained from the rotation matrices corresponding to the measurable rotation angles \(\alpha,\beta\), and \(\gamma\) of the pelvis plate around x,y, and z axes of \(\mathcal{F}\), respectively: 
\begin{equation} \label{eq:8}
\mathbf{R}_\mathcal{P}^\mathcal{F} = \mathbf{R}_x(\alpha)\mathbf{R}_x(\beta)\mathbf{R}_z(\gamma).
% \begin{bmatrix}
%c\beta\,c\gamma & -c\beta\,s\gamma & s\beta \\ s\alpha\,s\beta\,c\gamma + c\alpha\,s\gamma & -s\alpha\,s\beta\,s\gamma + c\alpha\,c\gamma & -\s\alpha\,c\beta \\ -c\alpha\,s\beta\,c\gamma + s\alpha\,s\gamma & c\alpha\,s\beta\,s\gamma + \s\alpha\,c\gamma & c\alpha\,c\beta
%\end{bmatrix}
\end{equation}
%with \(\alpha,\beta\) and \(\gamma\) as the measurable rotation angles of the pelvis plate with respect to the fixed frame around x,y and z axes, respectively.
%\item
The translation vector $\mathbf{T}_\mathcal{P}^\mathcal{O}$ is obtained using the summation of the following translations:
\begin{equation} \label{eq:5}
\mathbf{T}_\mathcal{P}^\mathcal{O} = \mathbf{T}_\mathcal{F}^\mathcal{O}+\mathbf{T}_\mathcal{P}^\mathcal{F}.
\end{equation}
%\end{itemize}


Note that the kinematic design of the hip-knee mechanism in Fig.~\ref{Fig:2}.a maintains the thigh link perpendicular to the closed-chain mechanism attachment at point \(M\), the thigh cannot rotate around its main axis. We can express the position of the revolute joint at \(M\) as:
\begin{equation} \label{eq:37}
\mathbf{T}_\mathcal{M}^\mathcal{O} = \mathbf{T}_\mathcal{H}^\mathcal{O} + \mathbf{R}_\mathcal{F}^\mathcal{O}\mathbf{R}_\mathcal{P}^\mathcal{F} \mathbf{R}_\mathcal{H}^\mathcal{P} 
\begin{bmatrix}
0 \\
0 \\
-l_m
\end{bmatrix},
\end{equation}
where $l_m$ is the thigh link segment length (which can be modified based on the user's thigh length). The rotational matrix associated with the hip is then:
\begin{equation} \label{eq:8b}
\mathbf{R}_\mathcal{H}^\mathcal{P} = \mathbf{R}_x(\theta_{fl})\mathbf{R}_y(\theta_{ab})\mathbf{R}_z(\theta_{ro}), 
% \begin{bmatrix}
% c\beta\,c\gamma & -c\beta\,s\gamma & s\beta \\ s\alpha\,s\beta\,c\gamma + c\alpha\,s\gamma & -s\alpha\,s\beta\,s\gamma + c\alpha\,c\gamma & -\s\alpha\,c\beta \\ -c\alpha\,s\beta\,c\gamma + s\alpha\,s\gamma & c\alpha\,s\beta\,s\gamma + \s\alpha\,c\gamma & c\alpha\,c\beta
% \end{bmatrix}
\end{equation} 
with $\theta_{fl}$, $\theta_{ab}$, and $\theta_{ro}$ the hip angles.

% On the other end, this closed-chain structure isattached to the thigh link of the orthosis via two perpendicular revolute joints (E and B).

Since the position of the revolute joint \(E\) is independent of the rotation of the revolute joint $M$, we can compute its position as:
\begin{equation} \label{eq:38}
\mathbf{T}_\mathcal{E}^\mathcal{O} = \mathbf{T}_\mathcal{H}^\mathcal{O} + \mathbf{R}_\mathcal{F}^\mathcal{O} \mathbf{R}_\mathcal{P}^\mathcal{F} \mathbf{R}_\mathcal{H}^\mathcal{P}
\begin{bmatrix}
0 \\
-l_n \\
-l_m
\end{bmatrix},
\end{equation}
where $l_m$ and $l_n$ are fixed segment lengths, with $l_n$ being the distance between the two non-actuated perpendicular revolute joints centered in \(E\) and \(B\) and $l_m$ defined above (see Fig.~\ref{Fig:2}).

%%%%%
\subsubsection*{\textbf{Prismatic actuators}}


From the actuator side, we can define a coordinate frame \(\mathcal{A}\) associated with the hip actuator plane (Fig.~\ref{Fig:2}.b), where the two linear actuators lie. This plane rotates by an angle \(\theta_A\) around the \(x\)-axis of the world frame \(\mathcal{O}\):
\begin{equation} \label{eq:9}
\mathbf{R}_\mathcal{A}^\mathcal{O} = \mathbf{R}_x(\theta_A).
 %\begin{bmatrix}
%1 & 0 & 0\\
 %0 & c\theta_A & -s\theta_A\\
%0 & s\theta_A & c\theta_A
%\end{bmatrix}
\end{equation}
%\subfile{KineStructure1}  %Note this file generates Fig. 3 (no text in the file)

From that, the positions of the distal ends of the shafts of the hip prismatic
actuators \(P_{ext}\) and \(P_{int}\) with respect to frame \(\mathcal{A}\) can be obtained using the following translational vectors: 


 \begin{equation} \label{eq:10}
\mathbf{T}^\mathcal{A}_{P_{ext}} =
 \begin{bmatrix}
\frac{1}{2}l_c \\
p_{ext} + d\\
0
\end{bmatrix}
\end{equation}
 \begin{equation} \label{eq:11}
\mathbf{T}^\mathcal{A}_{P_{int}} = 
 \begin{bmatrix}
-\frac{1}{2}l_c \\
p_{int} + d \\
0
\end{bmatrix}
\end{equation}
where \(l_c\) is the distance between the two parallel motors linear shafts, \(d\) is the distance between the rotation axis of the actuators and their foreheads, and \(p_{ext}\) and \(p_{int}\) represent how far the distal points of the motor on the shafts travel with respect to the actuator foreheads.  

% We can then define the position of \(E\) with respect to \({P_{ext}}\) and \({P_{int}}\) through the following translation matrices:

%  \begin{equation} \label{eq:12}
% \mathbf{T}^{P_{ext}}_E = \mathbf{R}^{P_{ext}}_E
%  \begin{bmatrix}
% 0 \\
% l_1\\
% 0
% \end{bmatrix},
% \end{equation}

%  \begin{equation} \label{eq:14}
%  \mathbf{T}^{P_{int}}_E = \mathbf{R}^{P_{int}}_E
%  \begin{bmatrix}
% 0 \\
% l_2\\
% 0
% \end{bmatrix},
% \end{equation}
% where:
% \begin{equation} \label{eq:13}
% \mathbf{R}^{P_{ext}}_E = \mathbf{R}_z(\theta_1),
% \end{equation}
% \begin{equation} \label{eq:15}
% \mathbf{R}^{P_{int}}_E = \mathbf{R}_z(-\theta_2).
% \end{equation}

The revolute joint point \(E\) in frame \(\mathcal{A}\) of the parallel mechanism can then be described as:

\begin{equation} \label{eq:16}
\mathbf{T}_\mathcal{E}^\mathcal{A} = \mathbf{T}_{P_{ext}}^\mathcal{A} + \mathbf{R}_z(\theta_1)
\begin{bmatrix}
0 \\
l_1\\
0
\end{bmatrix} = \mathbf{T}_{P_{int}}^\mathcal{A} + \mathbf{R}_z(-\theta_2)
\begin{bmatrix}
0 \\
l_2\\
0
\end{bmatrix}
\end{equation}
The rotation matrices \(\mathbf{R}_z(\theta_1)\) and \(\mathbf{R}_z(-\theta_2)\) are around z axis of \(\mathcal{A}\). The angles \(\theta_1\) and \(\theta_2\) with respect to the \(y\) axis of frame \(\mathcal{A}\) (see Fig.\ref{Fig:2}.b) can be easily obtained using basic trigonometric relationships.
Multiplying Eq.~\ref{eq:16} by \(\mathbf{R}_\mathcal{A}^\mathcal{O}\), the end-effector position of the revolute joint \(E\) can be obtained:
\begin{equation} \label{eq:39}
\mathbf{T}_\mathcal{E}^\mathcal{O} = \mathbf{R}_\mathcal{A}^\mathcal{O} \mathbf{T}_\mathcal{E}^\mathcal{A} =
\begin{bmatrix}
\frac{l_c}{2} - l_1 \sin \theta_1 \\
\cos \theta_A (p_{ext} + d + l_1 \cos \theta_1) \\
\sin \theta_A (p_{ext} + d + l_1 \cos \theta_1)
\end{bmatrix}.
\end{equation}
The position of the attaching point \(B\) of the thigh link of the orthosis with respect to the world frame is determined as:

\begin{equation} \label{eq:18}
\mathbf{T}^\mathcal{O}_\mathcal{B} = \mathbf{T}_\mathcal{E}^\mathcal{O} + \mathbf{R}_\mathcal{A}^\mathcal{O}\mathbf{R}_\mathcal{E}^\mathcal{A}\mathbf{R}_\mathcal{B}^\mathcal{E}
 \begin{bmatrix}
0 \\ 
l_n \\
0
\end{bmatrix},
\end{equation}
%
% \begin{equation} \label{eq:20}
% \mat{T}^A_B = \mathbf{T}_E^A + \mat{T}^E_B
% \end{equation}
where $\mathbf{R}_\mathcal{E}^\mathcal{A}$ according to the parallel mechanism is an identity matrix and $\mathbf{R}_\mathcal{B}^\mathcal{E} = \mathbf{R}_x(\theta_E)$, where \(\theta_E\) is the rotation of the revolute joint in \(E\) around x axis.
Considering \(\theta_B\) as the rotation angle of the second non-actuated revolute joint, \(B\), we can obtain the position of the hip joint with respect to the origin of the world frame as:
%therefore the position of hip joint respect to \(A\) is calculated through Eqs. (\ref{eq:21,23}).
% \begin{equation} \label{eq:21}
% \mathbf{T}^B_H = \mathbf{R}_H^B
%  \begin{bmatrix}
% 0 \\
% 0 \\ 
% l_m
% \end{bmatrix},
% \end{equation}
% where:
% \begin{equation} \label{eq:22}
% \mathbf{R}_H^B = \mathbf{R}_y(\theta_B)
% \end{equation}
% and:
% \begin{equation} \label{eq:23}
% \mathbf{T}^A_H = \mathbf{T}_B^A + \mathbf{T}^B_H.
% \end{equation}
% We can then derive the position of the hip joint \(H\) in the world frame \(\mathcal{O}\) as:
\begin{equation} \label{eq:24}
\mathbf{T}^\mathcal{O}_\mathcal{H} = \mathbf{T}^\mathcal{O}_\mathcal{B} + \mathbf{R}_\mathcal{A}^\mathcal{O}\mathbf{R}_\mathcal{E}^\mathcal{A}\mathbf{R}_\mathcal{B}^\mathcal{E}\mathbf{R}_\mathcal{H}^\mathcal{B}
\begin{bmatrix}
0 \\ 
0 \\
l_m
\end{bmatrix},
\end{equation}
where:
 \begin{equation} \label{eq:22}
\mathbf{R}_\mathcal{H}^\mathcal{B} = \mathbf{R}_y(\theta_B).
\end{equation}
Then, combining  Eq.~\ref{eq:24} with Eq.~\ref{eq:1}, the rotations \(\theta_A\), \(\theta_E\), and \(\theta_B\) can be derived.

\subsubsection*{\textbf{Closing the kinematic chain at the hip joint}}
By closing the kinematic chain in \(H\), we can extract the exoskeleton forward and inverse kinematic equations.
Moreover, considering that, if we define a coordinate frame \(\mathcal{H}\) fixed to the thigh segment, with its origin at point \(H\), we can express $\mathbf{R}_\mathcal{H}^\mathcal{P}$ also as:
\begin{equation} \label{eq:34}
\mathbf{R}_\mathcal{H}^\mathcal{P} = (\mathbf{R}_\mathcal{P}^\mathcal{F})^{-1} \mathbf{R}_\mathcal{H}^\mathcal{O} = 
\begin{bmatrix}
r_{11} & r_{12} & r_{13} \\
r_{21} & r_{22} & r_{23} \\
r_{31} & r_{32} & r_{33}
\end{bmatrix},
\end{equation}
where the rotation matrix of frame \(\mathcal{H}\) in frame \(\mathcal{O}\) is:
\begin{equation} \label{eq:33}
\mathbf{R}_\mathcal{H}^\mathcal{O} = \mathbf{R}_x(\theta_A) \mathbf{R}_x(\theta_E)\mathbf{R}_y(\theta_B) = 
\begin{bmatrix}
\vec{r}_{x'} & \vec{r}_{y'} & \vec{r}_{z'}.
\end{bmatrix}
\end{equation}
%In Eq.~\ref{eq:34}, 
and is obtained from:
\begin{itemize}
\item The vector \(\vec{EM}\), from point \(B\) to \(M\), defines the \(y'\)-axis:
\begin{equation} 
\vec{EM} = \mathbf{T}_\mathcal{M}^\mathcal{O} - \mathbf{T}_\mathcal{E}^\mathcal{O}
\end{equation}

\item The vector \(\vec{MH}\), from point \(M\) to hip joint \(H\), defines the \(z'\)-axis:
\begin{equation} 
\vec{MH} = \mathbf{T}_\mathcal{H}^\mathcal{O} - \mathbf{T}_\mathcal{M}^\mathcal{O}
\end{equation}

\item The \(x'\)-axis is computed as the cross product \(\vec{r}_{x'} = \vec{r}_{y'} \times \vec{r}_{z'}\), where \(\vec{r}_{y'}\) and \(\vec{r}_{z'}\) are the normalized vectors \(\vec{EM}\) and \(\vec{MH}\), respectively.
\end{itemize}

We can then use this to extract the hip angles as: 
\begin{equation}
\begin{split}
\theta_{fl} &= \arctan\left( \frac{-r_{23}}{r_{33}} \right) \\
\theta_{ab} &= \arcsin(r_{13}).
\end{split}
\label{eq:36}
\end{equation}
%\subsubsection*{\textbf{Validation of the model}}
The kinematic model of the mechanism was validated through an experiment performed by controlling the right leg of the exoskeleton in the execution of pre-recorded trajectories. Joint positions and angles obtained from the model were compared to those obtained from an OptiTrack\(^\text{\texttrademark}\) motion capture system (refer to the \textit{Supplementary materials} for details of the kinematic model validation process). 
%According to the results of the comparison, our kinematic model can accurately describe the positions and orientations of the joints of the robot. 

%\input{KinematicModel}

==> files/KineStructure1.tex <==
\begin{figure}
    \centering
%HV: please put in unit vectors of a frame that is in the plane of this system. So, instead of making this a top view (which would not be orthogonal to the plane of the actuators) just explicitly make this the plane of the actuators.
 %   \includegraphics[width=\columnwidth]{Actuators.png}
   % \caption{Top view of Actuators with parallel mechanism}





\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.38pt,y=0.38pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Straight Lines [id:da5169391076584446] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (489.39,58.26) -- (489.39,249.32) ;
%Shape: Can [id:dp8116292216370655] 
\draw  [color={rgb, 255:red, 219; green, 100; blue, 19 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (127.69,201.37) -- (127.72,146.99) .. controls (127.72,142.22) and (136.06,138.36) .. (146.35,138.36) .. controls (156.64,138.36) and (164.97,142.22) .. (164.97,146.99) -- (164.94,201.37) .. controls (164.94,206.14) and (156.6,210) .. (146.31,210) .. controls (136.02,210) and (127.68,206.14) .. (127.69,201.37) .. controls (127.69,196.61) and (136.03,192.75) .. (146.32,192.75) .. controls (156.61,192.75) and (164.95,196.61) .. (164.94,201.37) ;
%Shape: Can [id:dp7275326185322781] 
\draw  [color={rgb, 255:red, 219; green, 100; blue, 19 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (570.99,168.14) -- (559.36,168.14) .. controls (556.59,168.14) and (554.35,162.03) .. (554.35,154.51) .. controls (554.35,146.98) and (556.59,140.88) .. (559.36,140.88) -- (570.99,140.88) .. controls (573.76,140.89) and (576,146.99) .. (576,154.51) .. controls (576,162.04) and (573.76,168.14) .. (570.99,168.14) .. controls (568.22,168.14) and (565.97,162.04) .. (565.97,154.51) .. controls (565.97,146.98) and (568.22,140.88) .. (570.99,140.88) ;
%Shape: Can [id:dp18700508500995205] 
\draw  [color={rgb, 255:red, 219; green, 100; blue, 19 }  ,draw opacity=1 ][fill={rgb, 255:red, 255; green, 255; blue, 255 }  ,fill opacity=1 ] (472.99,183.7) -- (473.01,130.11) .. controls (473.02,126) and (480.21,122.67) .. (489.08,122.67) .. controls (497.95,122.67) and (505.14,126) .. (505.13,130.11) -- (505.11,183.7) .. controls (505.1,187.81) and (497.91,191.14) .. (489.04,191.14) .. controls (480.17,191.14) and (472.98,187.81) .. (472.99,183.7) .. controls (472.99,179.59) and (480.18,176.26) .. (489.05,176.26) .. controls (497.92,176.26) and (505.11,179.59) .. (505.11,183.7) ;
%Straight Lines [id:da5881118790399118] 
\draw    (488.86,115.97) -- (364.91,187.08) ;
%Straight Lines [id:da13432390764183588] 
\draw    (364.91,187.08) -- (364.91,265.25) ;
\draw [shift={(364.91,265.25)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(364.91,187.08)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da28256881084913266] 
\draw    (488.86,115.97) -- (488.86,194.14) ;
\draw [shift={(488.86,194.14)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(488.86,155.06)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(488.86,115.97)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da46351395040398646] 
\draw    (488.86,194.14) -- (364.91,265.25) ;
%Straight Lines [id:da7481242988654502] 
\draw    (280.5,112.72) -- (316.19,112.72) ;
%Straight Lines [id:da40367647189663614] 
\draw    (316.19,73.64) -- (316.19,151.8) ;
\draw [shift={(316.19,112.72)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da10316702850660664] 
\draw    (280.5,227.06) -- (364.91,226.16) ;
%Shape: Resistor [id:dp3202331274597021] 
\draw  [color={rgb, 255:red, 0; green, 0; blue, 0 }  ,draw opacity=1 ][fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (57.49,192.64) -- (231.54,192.64) -- (231.54,261.48) -- (57.49,261.48) -- (57.49,192.64) -- cycle (8.53,227.06) -- (57.49,227.06) (231.54,227.06) -- (280.5,227.06) ;
%Shape: Resistor [id:dp5016457792227524] 
\draw  [fill={rgb, 255:red, 155; green, 155; blue, 155 }  ,fill opacity=1 ] (57.46,78.16) -- (231.52,78.16) -- (231.52,147) -- (57.46,147) -- (57.46,78.16) -- cycle (8.51,112.58) -- (57.46,112.58) (231.52,112.58) -- (280.47,112.58) ;
%Straight Lines [id:da9046875490037485] 
\draw    (508,155) -- (554.35,154.51) ;
%Straight Lines [id:da8332976934626497] 
\draw [line width=1.5]  [dash pattern={on 5.63pt off 4.5pt}]  (146.51,46.51) -- (146.51,294.9) ;
%Straight Lines [id:da8332995062671782] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (617.71,153.6) -- (531.17,154.75) ;
%Straight Lines [id:da05432570628483191] 
\draw    (488.86,155.06) -- (316.19,112.72) ;
%Straight Lines [id:da46011885136501585] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (553.35,193.61) -- (491.86,194.12) ;
\draw [shift={(489.86,194.14)}, rotate = 359.52] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
\draw [shift={(555.35,193.59)}, rotate = 179.52] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da7959326151177646] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (554.35,154.51) -- (554.35,193.59) ;
\draw [shift={(554.35,193.59)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(554.35,174.05)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(554.35,154.51)}, rotate = 90] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da9114922691946221] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (451.44,264.09) -- (364.91,265.25) ;
%Straight Lines [id:da4221130975533365] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (402.73,111.56) -- (316.19,112.72) ;
%Shape: Arc [id:dp22831019720410928] 
\draw  [draw opacity=0] (359.46,112.14) .. controls (360.04,115.61) and (360.02,119.24) .. (359.31,122.88) -- (329.87,117.11) -- cycle ; \draw   (359.46,112.14) .. controls (360.04,115.61) and (360.02,119.24) .. (359.31,122.88) ;  
%Shape: Arc [id:dp16828507064475784] 
\draw  [draw opacity=0] (393.53,247.23) .. controls (395.82,250.12) and (397.62,253.5) .. (398.74,257.26) .. controls (399.6,260.12) and (400.01,263.01) .. (400.01,265.85) -- (370,265.85) -- cycle ; \draw   (393.53,247.23) .. controls (395.82,250.12) and (397.62,253.5) .. (398.74,257.26) .. controls (399.6,260.12) and (400.01,263.01) .. (400.01,265.85) ;  
%Straight Lines [id:da3829268754366655] 
\draw [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ]   (146.51,170.71) -- (146.42,216.95) ;
\draw [shift={(146.41,219.95)}, rotate = 270.11] [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(146.51,170.71)}, rotate = 90.11] [color={rgb, 255:red, 208; green, 2; blue, 27 }  ,draw opacity=1 ][fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da7064578522868845] 
\draw [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ]   (146.51,170.71) -- (203.05,171.31) ;
\draw [shift={(206.05,171.34)}, rotate = 180.61] [fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=1 ][line width=0.08]  [draw opacity=0] (8.93,-4.29) -- (0,0) -- (8.93,4.29) -- cycle    ;
\draw [shift={(146.51,170.71)}, rotate = 0.61] [color={rgb, 255:red, 144; green, 19; blue, 254 }  ,draw opacity=1 ][fill={rgb, 255:red, 144; green, 19; blue, 254 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da7958170312482791] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (43.46,114.58) -- (43.49,225.06) ;
\draw [shift={(43.49,227.06)}, rotate = 269.99] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
\draw [shift={(43.46,112.58)}, rotate = 89.99] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da054662996260238295] 
\draw  [dash pattern={on 0.84pt off 2.51pt}]  (229.54,273.07) -- (149,273.57) ;
\draw [shift={(147,273.58)}, rotate = 359.65] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
\draw [shift={(231.54,273.06)}, rotate = 179.65] [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.08]  [draw opacity=0] (12,-3) -- (0,0) -- (12,3) -- cycle    ;
%Straight Lines [id:da8025827459982644] 
\draw  [dash pattern={on 4.5pt off 4.5pt}]  (231.54,227.06) -- (231,299) ;
%Straight Lines [id:da6455049988431105] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (316.19,112.72) ;
\draw [shift={(316.19,112.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(316.19,112.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da7837221179724421] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (365.19,225.72) ;
\draw [shift={(365.19,225.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(365.19,225.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da7577864734406472] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (147.19,170.72) ;
\draw [shift={(147.19,170.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(147.19,170.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da7880590860194232] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (489.19,154.72) ;
\draw [shift={(489.19,154.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(489.19,154.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
%Straight Lines [id:da2940726592353988] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (554.19,154.72) ;
%\draw [shift={(574.19,154.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;
\draw [shift={(574.19,154.72)}, rotate = 0] [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ][line width=0.75]      (0, 0) circle [x radius= 3.35, y radius= 3.35]   ;


% Text Node
\draw (295.42,211) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.29,0.56,0.89}{p_{ext}}$};
% Text Node
\draw (273.42,97) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.29,0.56,0.89}{p_{int}}$};
% Text Node
\draw (188.42,288) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.29,0.56,0.89}{d}$};
% Text Node
\draw (28.42,169) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.29,0.56,0.89}{l_c}$};
% Text Node
\draw (110,170) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.96,0.65,0.14}{A}$};
% Text Node
\draw (214,155) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.56,0.07,1}{y-z}$};
% Text Node
\draw (136,210) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.82,0.01,0.11}{x}$};
% Text Node
\draw (497,143) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.96,0.65,0.14}{E}$};
% Text Node
\draw (583,133) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.96,0.65,0.14}{B=M}$};
% Text Node
\draw (362.42,135) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\theta _{2}$};
% Text Node
\draw (413.42,254) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\theta _{1}$};
% Text Node
\draw (527.42,211) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.29,0.56,0.89}{l}\textcolor[rgb]{0.29,0.56,0.89}{_{n}}$};
% Text Node
\draw (415.42,125) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.29,0.56,0.89}{l}\textcolor[rgb]{0.29,0.56,0.89}{_{2}}$};
% Text Node
\draw (436.42,240) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.29,0.56,0.89}{l}\textcolor[rgb]{0.29,0.56,0.89}{_{1}}$};
% Text Node
\draw (383.42,218) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.96,0.65,0.14}{P_{ext}}$};
% Text Node
\draw (335.42,97) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\textcolor[rgb]{0.96,0.65,0.14}{P_{int}}$};
% Text Node
\draw (647.42,152) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\theta _{B}$};
% Text Node
\draw (490.42,34) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\theta _{E}$};
% Text Node
\draw (145.42,24) node  [font=\large,color={rgb, 255:red, 0; green, 0; blue, 0 }  ,opacity=1 ,rotate=-359.76]  {$\theta _{A}$};


\end{tikzpicture}
    \caption{Hip actuators with parallel mechanism in actuator plane; The x-axis is placed on x-axis of origin and y-z axis is a unit vector in y-z plane of origin with parallel mechanism. \(l_c\) is the distance between the two parallel motors' linear shafts, \(d\) is half the length of the linear actuators, and \(P_{ext}\) and \(P_{int}\) represent how far the motor shafts travel. $\theta _{A}$, $\theta _{B}$, and $\theta _{E}$ are unknowns.}
    \label{Fig:3}
\end{figure}

==> files/Methods_old.tex <==
\section{Methods}
\subsection{The treadmill-based lower-limb exoskeleton}
\label{Sec:loko}
For this work, we used a grounded exoskeleton developed at the Sensory Motor Systems (SMS) Lab at ETH Zurich in collaboration with Hocoma AG, Switzerland (Fig.~\ref{fig:experimental_setup}). The new exoskeleton is a modified version of the company's well-known Lokomat\textsuperscript{\textregistered}. In particular,
the system maintains the original Lokomat\textsuperscript{\textregistered}, parts of the body-weight support (BWS) system, the treadmill, and the knee joint flexion/extension ball-screw-driven linear actuation. The system also maintains the in-line force sensor at the knee actuation to measure the human-robot force interaction\cite{lokomatPro2023}. 

The mechanical innovations of the modified exoskeleton include: i) changes in the hip actuation to allow for hip flexion/extension and ab-/adduction~\cite{wyss2019}, ii) a pelvis module that embodies a six degree of freedom (DoF) compliant mechanism that accommodates weight shifting during walking, with one actuated DoF that assists the pelvis lateral movements~\cite{wyss2018multidimensional}, and iii) the original BWS system augmented by one actuated DoF that enables lateral movements to follow the pelvis lateral movements~\cite{wyss2014body}.  
These innovations resulted in a human–exoskeleton interface that incorporates twelve degrees of freedom (DoFs): six at the pelvis, two at each hip, and one at each knee. Among these, seven DoFs are actuated: one at the pelvis (coupled with the new actuated BWS lateral mechanism), two at each hip (flexion/extension and ab-/adduction), and one at each knee. Fig.~\ref{Fig:2}.a represents the full kinematic model of the right leg.
\begin{figure}[ht!]
    \centering
    \includegraphics[width=\linewidth]{figures/lokom1.png}
    \caption{(a) The new exoskeleton with a user secured, featuring an active body weight support (BWS) system with actuated lateral movement capability, a 6-DoF series elastic actuation (SEA) pelvis module with additional lateral translation actuator, two active 2-DoF closed-chain hip actuators, ball-screw-driven 1-DoF knee actuators, ankle/shank/thigh cuffs, and a safety harness for fall prevention. (b) Detail of the 6-DoF pelvis module. (c) Detail of the closed-chain mechanism for hip actuation.}
    \label{fig:experimental_setup}
\end{figure}

The \textbf{pelvis module} includes a pelvis plate, centered at point \(P\) in  Fig.~\ref{Fig:2}.a, which is attached to the user's pelvis and can undergo both translational and rotational motion with respect to frame \(\mathcal{F}\). This is achieved by a compliant spring-based connection between the fixed back of the pelvis module and the pelvis plate (Fig.~\ref{fig:experimental_setup}.b; see~\cite{wyss2019} for further details). The pelvis module functions as a series elastic actuator (SEA), with one actuated degree of freedom (P01-48x240 motor, NTI AG LinMot, Switzerland), enabling lateral movement relative to a fixed frame. To prevent hindering the natural lateral movement of the pelvis, the BWS is laterally actuated through a lead-screw mechanism parallel to the pelvis's actuated degree of freedom. Note that the other parts of the BWS remain unchanged with respect to their commercial version, i.e., allow for static and dynamic users' weight unloading. 

\textbf{Hip actuation} is achieved through a closed-chain mechanism (Fig.~\ref{fig:experimental_setup}.c) driven by two linear actuators per leg (P01-48x240 motors, LinMot, Switzerland). The two prismatic actuators per leg are located on a plane that can rotate around the x-axis of the global frame \(\mathcal{O}\) (see Fig.~\ref{Fig:2}.a). 
This configuration enables control of both hip flexion/extension and ab-/adduction, while maintaining a rigid joint rotation. %
\subfile{KineStructure}%
This is achieved through a parallel closed-chain mechanism connected to the outputs of two joints (denoted by $P_{int}$ and $P_{ext}$ in Fig.~\ref{Fig:2}.a) located at the distal end of the shafts of the hip prismatic actuators. On the other end, this closed-chain structure is attached to the thigh link of the orthosis via two perpendicular revolute joints ($E$ and $B$ in Fig.~\ref{Fig:2}.a). 
This mechanism converts the independent translational motions of the linear actuators into coordinated movements of the thigh link in the frontal and sagittal planes, as illustrated in Fig.~\ref{fig:hip-model}. In particular, this configuration enforces hip flexion/extension movements when the two linear actuators move in the same direction (Fig.~\ref{fig:hip-model}.b), while ab-/adduction movements are produced by moving in opposite directions (Fig.~\ref{fig:hip-model}.c). By allowing the linear actuators to rotate about the x-axis of the passive joint $A$, the system avoids overconstraining the leg. 


In Fig.~\ref{Fig:2}.a, the thigh rotational motion is represented by three rotational axes intersecting in $H$. Note that the hip internal/external rotation is mechanically constrained by the exoskeleton’s structure and, aside from small contributions from pelvis rotation, remains approximately fixed. 

This mainly parallel actuation configuration offers several benefits over a serial approach like the FreeD, the most notable being a reduction in orthosis inertia, resulting in a more transparent system by design. % resulting  the robot a versatile system able to provide either stiff or compliant control.

For completeness, Fig.~\ref{Fig:2}.a also includes the \textbf{knee joint}, which is part of the original Lokomat\textsuperscript{\textregistered} device. The knee joint is located at the distal end of the thigh link, connected to the closed-chain structure via a revolute joint ($K$) and provided with a built-in force sensor. 

The various actuators have built-in incremental 
position encoders. The pelvis module includes a Pixart infrared (IR) motion camera (PixArt Imaging Inc., Hsinchu, Taiwan) and a 6-DoF inertial measurement unit (IMU)(MPU9250, InvenSense, San Jose, USA). A Kalman filter is used to combine the IMU and camera data to estimate the position and orientation of the pelvis plate with respect to the fixed back of the pelvis module, see~\cite{wyss2019} for further details. 

The exoskeleton is attached to the participant's lower limbs using the Lokomat\textsuperscript{\textregistered} original cuffs placed on the thighs, shanks, and ankles. The participant's pelvis is secured to the pelvis module between two house-made fixtures positioned on either side, as shown in Fig.\ref{fig:experimental_setup}.a. 
Additionally, participants wear a body harness suspended on the BWS. 



%As per the control unit, the robot is controlled via MATLAB Simulink Real-Time 2013, operating at a control frequency of \SI{500}{Hz}. We developed a SimMechanics model of the system using MATLAB\textsuperscript{\textsuperscript{\textregistered}} Simscape Multibody (R2021b, MathWorks, USA).

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.78\columnwidth]{figures/fig-model2.pdf}
    \caption{Top view of the right leg's closed-chain mechanism with the pelvis fixed in rotation, shown in different configurations: a) Neutral, b) Hip flexion/extension motion, and c) Hip ab-/adduction motion. Orange and purple arrows represent the movement of the linear actuators. Red and green arrows represent the resulting motion at the thigh.}
    \label{fig:hip-model}
    \vspace{-0.3cm}
\end{figure}
 
\subsection{Exoskeleton kinematic model}
\label{sec:kine}

We developed a closed-form analytical solution for the forward and inverse kinematics of the robot hip actuator module to be able to enforce personalized joint trajectories.
Since the mechanism does not incorporate any sensors to measure the rotations of the hip joint at $H$, we determined the direct and inverse mapping between the actuators' joint coordinates ($p_{int}$, $p_{ext}$, Fig.~\ref{Fig:2}.b) representing the shaft length of the two prismatic actuators of the hip module, and the space of hip joint coordinates ($\theta_{fl}$, $\theta_{ab}$, and $\theta_{ro}$, Fig.~\ref{Fig:2}.a), representing the hip flexion/extension, ab-/adduction, and internal/external rotation, respectively.

In the following paragraphs, we present the kinematic model and the process we followed for its definition, consisting of building the structure from both the perspective of the pelvis plate and the linear actuators to the spherical hip joint of the exoskeleton, and then closing the kinematic chain. 
Position and orientation of each joint will be expressed using homogeneous transformation matrices relative to the origin frame, \(\mathcal{O}\). In the following equations, \(\mathbf{T}_\mathcal{X}^\mathcal{Y}\) represents the translation vector from frame \(\mathcal{Y}\) to frame \(\mathcal{X}\), expressed in frame \(\mathcal{Y}\) coordinates, and \(\mathbf{R}_\mathcal{X}^\mathcal{Y}\) denotes the rotation matrix describing the orientation of frame \(\mathcal{X}\) relative to frame \(\mathcal{Y}\).


%\subsection{Kinematic loop-closure formulation}

The hip module of the exoskeleton forms a closed kinematic chain that can be expressed by closing two branches of the loop, either at the hip joint $H$ or at the upper hinge $E$ of the parallel mechanism (see Fig.~\ref{Fig:2}a). In the following, we derive the homogeneous positions of $H$ and $E$ from both closed-loop branches.

\subsubsection{Top branch (O $\rightarrow H \rightarrow M \rightarrow E$)}
The pelvis plate pose is defined by its measured rotations $\alpha,\beta,\gamma$, respect to fixed frame, around x,y and z axes respectively:
\begin{equation}
R^\mathcal{F}_\mathcal{P} = R_x(\alpha)R_y(\beta)R_z(\gamma), \qquad
T^\mathcal{O}_\mathcal{P} = T^\mathcal{O}_\mathcal{F} + T^\mathcal{F}_\mathcal{P} .
\end{equation}
The hip joint $H$, rigidly mounted on the pelvis plate, is located at a calibrated offset $T^\mathcal{P}_\mathcal{H}$ to be adaptable to accommodate different user sizes:
\begin{equation}
T^\mathcal{O}_\mathcal{H}\big|_{\text{top}} = T^\mathcal{O}_\mathcal{P} + R^\mathcal{F}_\mathcal{P} T^{P}_{H} .
\end{equation}
where the index \textit{top} indicates the propagation along the top branch.
The hip orientation in $O$ is given by
\begin{equation}
R^\mathcal{O}_\mathcal{H} = R^\mathcal{F}_\mathcal{P} R^\mathcal{P}_\mathcal{H}, \qquad
R^\mathcal{P}_\mathcal{H} = R_x(\theta_{fl})R_y(\theta_{ab})R_z(\theta_{ro}) .
\end{equation}
Propagating along the thigh yields
\begin{equation}
T^\mathcal{O}_\mathcal{E}\big|_{\text{top}} = T^\mathcal{O}_\mathcal{H}\big|_{\text{top}} + R^\mathcal{O}_\mathcal{H}
\begin{bmatrix}
0 \\ -l_n \\ -l_m
\end{bmatrix}.
\end{equation} 

\subsubsection{Bottom branch ($O \rightarrow E \rightarrow B \rightarrow H$)}
The actuator plane $A$ is rotated by $\theta_A$ about the $x$-axis:
\begin{equation}
R^\mathcal{O}_\mathcal{A} = R_x(\theta_A).
\end{equation}
The distal ends of the linear actuators are:
\begin{equation}
T^\mathcal{A}_{P_{\mathrm{ext}}} =
\begin{bmatrix}
\frac{l_c}{2} \\ p_{\mathrm{ext}} + d \\ 0
\end{bmatrix}, \quad
T^\mathcal{A}_{P_{\mathrm{int}}} =
\begin{bmatrix}
-\frac{l_c}{2} \\ p_{\mathrm{int}} + d \\ 0
\end{bmatrix}.
\end{equation}
With link orientations $R^\mathcal{A}_{P_{\mathrm{ext}}E} = R_z(\theta_1)$ and $R^\mathcal{A}_{P_{\mathrm{int}}E} = R_z(-\theta_2)$, the hinge $E$ satisfies:
\begin{equation}
T^\mathcal{A}_\mathcal{E} = T^\mathcal{A}_{P_{\mathrm{ext}}} + R^\mathcal{A}_{P_{\mathrm{ext}}E}
\begin{bmatrix}0\\l_1\\0\end{bmatrix}
= T^\mathcal{A}_{P_{\mathrm{int}}} + R^\mathcal{A}_{P_{\mathrm{int}}E}
\begin{bmatrix}0\\l_2\\0\end{bmatrix}.
\label{eq:TA_E}
\end{equation}

Multiplying Eq.~\ref{eq:TA_E} by \(\mathbf{R}_A^O\), the  position of the revolute joint \(E\) can be obtained:
\begin{equation}
T^\mathcal{O}_\mathcal{E}\big|_{\text{bot}} = R^\mathcal{O}_\mathcal{A} T^\mathcal{A}_\mathcal{E} =
\begin{bmatrix}
\frac{l_c}{2} - l_1 \sin \theta_1 \\
\cos \theta_A (p_\mathrm{ext} + d + l_1 \cos \theta_1) \\
\sin \theta_A (p_\mathrm{ext} + d + l_1 \cos \theta_1)
\end{bmatrix}.
\end{equation}
where the index \textit{bot} indicates the propagation through the bottom branch. Propagating further along the bottom branch:
\begin{align}
T^\mathcal{O}_\mathcal{B} &= T^\mathcal{O}_\mathcal{E}\big|_{\text{bot}} + R^\mathcal{O}_\mathcal{A} R_x(\theta_E)
\begin{bmatrix}0\\ l_n \\ 0\end{bmatrix}, \\
T^\mathcal{O}_\mathcal{H}\big|_{\text{bot}} &= T^\mathcal{O}_\mathcal{B} + R^\mathcal{O}_\mathcal{A} R_x(\theta_E) R_y(\theta_B)
\begin{bmatrix}0\\ 0\\ l_m\end{bmatrix}.
\end{align}

\subsubsection{Loop-closure conditions}
To solve for the unknown variables, the loop-closure equations are formulated by equating the two branches of the mechanism. 
The kinematic loop can be closed either at the hip joint ${H}$ or at the upper hinge ${E}$ of the parallel mechanism:
\begin{align}
&\text{Closure at $H$:} & T^\mathcal{O}_\mathcal{H}\big|_{\text{top}} &= T^\mathcal{O}_\mathcal{H}\big|_{\text{bot}} , \\
&\text{Closure at $E$:} & T^\mathcal{O}_\mathcal{E}\big|_{\text{top}} &= T^\mathcal{O}_\mathcal{E}\big|_{\text{bot}} .
\end{align}
Both systems of equations yield a valid solution to the closed-loop kinematics. 
The first formulation, closed at $H$, is particularly convenient for \textit{forward kinematics} (joint $\rightarrow$ actuator space), whereas the second, closed at $E$, is more convenient for \textit{inverse kinematics} (actuator $\rightarrow$ joint space).


The kinematic model of the mechanism was validated through an experiment performed by controlling the right leg of the exoskeleton in the execution of pre-recorded trajectories. Joint positions and angles obtained from the model were compared to those obtained from an OptiTrack\(\textsuperscript{\texttrademark}\) motion capture system. We refer the reader to the \textit{Supplementary Materials} for details of the kinematic model validation process. 


\subsection{Gait pattern prediction models}
\label{sec:model}

We developed models to predict leg joint and pelvis trajectories based on individual characteristics such as height and age. Our approach builds on the models proposed by Koopman \textit{et al.} \cite{koopman2014}, which use multiple polynomial regression models to predict knee and hip flexion/extension joint trajectories from a person's height and walking speed. To improve the personalization potential of Koopman's proposed models, here we also account for the effect of other factors (e.g., age, body weight, and gender), which have been shown to substantially affect joint angles and overall walking patterns~\cite{oberg1994,hanlon2006,wu2018,ren2019}. 
We further expanded the model to predict the trajectories of the augmented DoFs of our exoskeleton, namely, the lateral pelvis translation and hip ab-/adduction.

%Alongside the models to predict personalized joint trajectories, we also defined a Standard Gait Pattern, meant to providea standard pattern ideally suitable for all participants.
%Following Koopman’s approach, we used regressions to predict a sparse set of key points—called key events, namely —along each joint trajectory, rather than the full time series. We are following the same concept for our approach: for each key event, the model estimates time, joint angle or displacement, velocity, and acceleration. These events are spaced to capture the trajectory’s overall shape, allowing full personalized gait patterns to be reconstructed through interpolation.

\subsubsection*{\textbf{Database}}
\label{sec:database}
To train and validate our model, we used the publicly available gait database from the Laboratory of Biomechanics and Motor Control at the Federal University of ABC, Brazil~\cite{fukuchi2018}. This database includes data from \SI{42}{}~volunteers, split into \SI{24}{}~young adults (\SIrange{21}{37}{years}) and \SI{18}{}~older adults (\SIrange{50}{84}{years}), all without lower-extremity injuries or gait impairments. Data were collected with a marker-based motion-capture system composed of twelve cameras, from participants walking barefoot on a treadmill at eight different speeds, ranging from \SI{40}{\%} to \SI{145}{\%} of their comfortable, self-selected walking speed.
Table~\ref{tab:anthropometric_demographic_data} summarizes the anthropometric and demographic characteristics of this dataset. Compared to the database used by Koopman \textit{et al.}, which included gait kinematics from fifteen middle-aged participants, this dataset encompasses a broader range of subjects, including individuals in their twenties up to nearly \SI{80}{years} old.

\begin{table}[ht!]
\centering
\caption{Descriptive statistics of participants' anthropometric and demographic data from~\cite{fukuchi2018} used to train our predictive models}
\begin{tabular}{lllll}
\toprule
Parameter   & Mean   & Std.  & Min  & Max  \\ \midrule
Age (years) & 42.64  & 18.62 & 21   & 84   \\
Height (cm) & 167.12 & 11.01 & 147  & 192  \\
Mass (kg)   & 67.76  & 11.24 & 44.9 & 95.4 \\ \bottomrule
\end{tabular}
\label{tab:anthropometric_demographic_data}
\end{table}

The dataset includes both raw---e.g., marker coordinates and external forces---and processed data---e.g., knee and hip flexion/extension and hip ab-/adduction joint trajectories for each participant at recorded speed level. The database did not include the processed data regarding the lateral pelvis trajectories, so we derived them from the raw marker trajectories. 
All joint trajectories, including the newly computed lateral pelvis movement, were represented as time-normalized ensemble averages for each participant at their respective gait speeds.

While the database included treadmill speeds up to \SI{8.02}{\kilo\metre\per\hour}, our treadmill has a speed limit of \SI{3.2}{\kilo\metre\per\hour} \cite{lokomatPro2023}. Therefore, only a subset of the speeds recorded in the original database was included for training our gait pattern prediction model, namely:
\begin{itemize}
    \item Level 1, \SI{40}{\%} of self-selected speed: $1.80\pm$ \SI{0.231} {\kilo\metre\per\hour};
    \item Level 2, \SI{55}{\%} of self-selected speed:  $2.46\pm$\SI{0.336}{\kilo\metre\per\hour};
    \item Level 3, \SI{70}{\%} of self-selected speed: $3.14\pm$\SI{0.410}{\kilo\metre\per\hour}.
\end{itemize}   
 

\begin{figure*}[ht!]
    \centering
    % First row: three plots side by side
    \begin{subfigure}{}
        \includegraphics[width=0.45\linewidth]{figures/hipAbductionKEs1.png}
    \end{subfigure}%
    \begin{subfigure}{}
        \includegraphics[width=0.45\linewidth]{figures/hipFlexionKEs1.png}
    \end{subfigure}
    \vspace{0.5cm} \\
    
    % Second row: one plot
    \begin{subfigure}{}
        \includegraphics[width=0.45\linewidth]{figures/kneeFlexionKEs1.png}
    \end{subfigure}%
    \begin{subfigure}{}
        \includegraphics[width=0.45\linewidth]{figures/latPelvisMoveKEs1.png}
    \end{subfigure}

    \caption{Exemplary right leg trajectories of a participant are displayed at walking speed levels 1, 2, and 3, together with their extracted key events. These key events are the same as in Koopman's study \cite{koopman2014}, except for lateral pelvis movement (not present in their study), for which extreme position and velocity values were chosen. The key events for the left and right joint trajectories were extracted separately. By default, heel strike timing is set to zero (\% of the gait cycle), as are the minimum and maximum values for joint position and velocity. These constraints are detailed in the key event legend.}
    \label{fig:key_events_example}
\end{figure*}

\subsubsection*{\textbf{Prediction models for gait key events}}
\label{sec:reg_training}

Following Koopman \textit{et al.} approach, we used regression models to predict a sparse set of key points within the joint trajectories, called key events. 
These events are spaced to capture the trajectory’s overall shape, allowing full personalized gait patterns to be reconstructed through interpolation. From the hip and knee trajectories, six key events each were selected, namely the start of the joint trajectory (heel contact) and the maximum values in position and velocity during both swing and stance phases
~\cite{koopman2014}. 
For the lateral pelvis movement, only four key events were employed, corresponding to the point of maximum and minimum pelvis position and velocity along the trajectory. 
Each event is defined as a set of four parameters: (i) timing ($t$) expressed as a percentage of the gait cycle, (ii) angle or displacement ($y$), (iii) (angular) velocity ($\dot{y}$), and (iv) acceleration ($\ddot{y}$); see Fig.~\ref{fig:key_events_example} for exemplary right leg trajectories with key events of a single participant at the three walking speed levels. 

We trained regression models to predict each of these four parameters, which were then used to reconstruct the final personalized trajectories. We employed the following initial main regression equation:
\begin{equation}
\label{eq:main}
Y = \beta_c + \beta_v v + \beta_{v^2}v^2 + \beta_hh + \beta_ww + \beta_aa + \beta_ss,
\end{equation}
where $v$ represents walking speed, $h$ body height, $w$ body weight, $a$ age, and $s$ gender, encoded as a numerical value where female is $-1$ and male is $1$. The output $Y$ represents the predicted key event parameter, i.e., time ($t$), position ($\theta$), velocity ($\dot{y}$), or acceleration ($\ddot{y}$).

We fit one regression model per parameter for all the key events, leading to 24 regression models for each hip ab-/adduction, hip flexion/extension, and knee flexion/extension trajectory (i.e., four parameters per each of the six key events per trajectory), and 16 models for the lateral pelvis movement (with only four key events). To prevent overfitting and improve interpretability, stepwise regression was conducted to evaluate the significance of the predictor variables in Eq.~\ref{eq:main}. Only variables with significant effects ($p < 0.01$) were retained, following the Koopman \textit{et al.} approach~\cite{koopman2014}. Then, robust regressions with a \textit{bisquare} weighting function were employed to estimate the final regression coefficients ($\beta_x$). In this way, different models could rely on different predictors (see the \textit{Supplementary Materials} for the complete regression equations derived for the different joint trajectories).


An additional regression model was derived from Eq.~\ref{eq:main} to predict the gait cycle time, resulting in:
%
\begin{equation}
\label{equa:regression_equation_cycle_time}
T_{pre} =  2.7662 - 0.7458v + 0.0903v^2  - 0.0037a, 
\end{equation}
%
where the gait cycle time ($T_{pre}$) depends on the walking speed ($v$) and age ($a$).




\subsubsection*{\textbf{Generation and evaluation of Personalized Gait Patterns based on predicted key events}}

From the predicted four parameters of each gait key event (i.e., $t$, $y$, $\dot{y}$, or $\ddot{y}$), we then generated personalized continuous joint kinematic trajectories. We employed the 5th-order piece-wise quintic splines interpolation method, as proposed by Koopman \textit{et al.}~\cite{koopman2014}.


The accuracy of the predicted trajectories was evaluated using the data from the publicly available database \cite{fukuchi2018}. We computed the root mean square error (RMSE) against the real database trajectories, using the leave-one-out cross-validation method. The results were then averaged across all participants and over both left and right joint trajectories.

% The RMSE is defined as follows:
% \begin{equation}
% RMSE = \sqrt{\frac{\sum_{t=1}^{N} (y_t - \hat{y}_t)^2}{N}}.
% \label{equation:RMSE}
% \end{equation}
% Here, $N$ represents the number of data points in the gait cycle (101 time-normalised points), $y_t$ corresponds to the actual joint angle/displacement value at time $t$, and $\hat{y}_t$ denotes the corresponding predicted value. %This evaluation method allows for a quantitative assessment of the performance of the gait prediction model in terms of accuracy in predicting gait patterns.



\subsubsection*{\textbf{Generation and evaluation of the \textit{Standard Gait Pattern}}}

Alongside the \textit{Personalized Gait Pattern}, we used the same database to define a \textit{Standard Gait Pattern}, meant to provide a standard pattern ideally suitable for all participants. This standard pattern was obtained by averaging the gait patterns of the three included walking speed levels across all participants in the dataset. We globally assumed symmetrical gaits, so the trajectories of both the left and right legs were combined. Note that this average was taken over the entire trajectory, rather than averaging over the key events. 

Because this was conceived as a standard gait pattern for all scenarios, we, therefore, had to adjust the trajectories by estimating the gait cycle time ($T_{stand}$) to account for different desired gait speeds. Therefore, a regression model, reduced following the same steps described above, was employed to estimate the gait cycle time also for the \textit{Standard} gait pattern: 
%
\begin{equation}
\label{equa:regression_formula_cycle_time_standard}
\begin{aligned}
T_{stand} = \ & 1.8993 - 0.6909v + 0.0789v^2 + 0.3928h. %
\end{aligned}
\end{equation}

We calculated the RMSEs between the standard and actual gait patterns from the database 
as a means to compare their accuracy with that from the \textit{Personalized} gait pattern.




\subsection{Pilot user evaluation of the Personalized and Standard gait patterns}
\label{sec:experiment}
\subsubsection*{\textbf{Participants}}
Ten unimpaired participants participated in the pilot study, equally divided into females and males. Their ages ranged from \SIrange{23}{27}{years}, with a mean age of $25$ years, average height of $1.76\pm$\SI{0.089}{\meter}, and weight of $69.25\pm$\SI{12.79}{\kilo\gram}. None reported neurological or orthopaedic disorders. 
%
%
%\subsubsection*{\textbf{Experimental protocol}}
The study was approved by our university's Ethics Committee. Prior to the experiment, all participants read and signed an informed consent form. % (application date: 25.08-2023). 

\subsubsection*{\textbf{Experimental protocol}}
Participants underwent three different test conditions (trials), of two minutes each, with the exoskeleton guiding their lower limbs along three distinct gait patterns: (i) the \textit{Personalized} gait pattern, (ii) the \textit{Standard} gait pattern, and (iii) a \textit{Random} gait pattern. The first two gait patterns were introduced in detail in Sec.\ref{sec:reg_training}. In the \textit{Random Gait Pattern} condition, participants were guided to follow a gait pattern randomly selected (for each participant) from the recorded patterns from Fukuchi's database \cite{fukuchi2018}. 
The inclusion of this random pattern
served as a baseline to observe the effects of potentially mismatched, non-tailored assistance in comparison with more personalized ones.
The order of the gait pattern condition trials was pseudo-randomized across participants, i.e., each of the six possible condition sequences was used once (following a Latin square), and then four more sequences were randomly selected from these six.


Participants were instructed to remain passive to the movement of the exoskeleton and received no indication about the differences among gait pattern conditions. We operated the exoskeleton in Proportional-Derivative (PD) control, with the computed gait patterns as reference trajectories. The controller was intentionally rigid (for the hip and pelvis PD controller: $Kp =$\,\SI{5.0}{\ampere\per\milli\meter} and $Kd =$\,\SI{7.5}{\ampere\per(\meter\per\second)}, for the knee PD controller: $Kp =$\,\SI{1.0}{\ampere\per\milli\meter} and $Kd =$\,\SI{0.1}{\ampere\per(\meter\per\second)}), allowing minimal compliance to enhance the user's sensitivity to variations in gait patterns. We also aimed to achieve stiff connection points between the participants' limbs and the robotic device at the pelvis, thighs, and shanks to make trajectory differences more perceptible to the participants. Yet, we acknowledge that the soft tissue of participants' limbs, together with the Velcro\textsuperscript{\textregistered} straps used at the human-robot interaction points, might have introduced some compliance in the connection. While participants were wearing the harness, the BWS system remained slack, such that participants did not receive any weight compensation.


For all conditions, the walking speed was set to \SI{1.8}{\kilo\metre\per\hour}, reflecting the average speed of the lowest walking speed level in the database. Therefore, the random gait pattern was selected only from the pool of patterns in the lowest walking speed level, i.e., Level 1 in Sec.\ref{sec:database}. Only for some participants, who explicitly requested to increase the speed to walk more comfortably, it was set to  \SI{2.0}{\kilo\metre\per\hour}. % The walking speed for the random patterns varied around the target speed of \SI{1.8}{\kilo\metre\per\hour}, with a standard deviation of $\pm$\SI{0.231}{\kilo\metre\per\hour}. 



After signing the informed consent form, participants wore the exoskeleton, which was adjusted to each of their body dimensions, including the width of the pelvis, the frontal position of the hip joint, thigh length, and shank length. The kinematic model (see Fig.~\ref{Fig:2}) was adjusted according to these dimensions. The reference actuator position trajectories were then generated using the exoskeleton model and based on hip ab-/adduction, hip flexion/extension, and pelvis lateral motion calculated patterns. Once the exoskeleton was fit and the exoskeleton kinematic model adjusted, participants underwent a familiarization phase before testing the three different gait pattern conditions. During this initial phase, participants walked with the exoskeleton in a `transparent mode'~\cite{marchalCrespo2009}, i.e., they could move as freely as possible while getting used to walking with the exoskeleton. %To ensure safety, participants wore a harness, but no body weight support was provided. 
Emergency stops were provided to both the participant and the experimenter.





\subsubsection*{\textbf{Data acquisition and processing}}

%\subsubsection{User experience}
After each condition, participants filled in a questionnaire to evaluate their perceptions of the different gait pattern conditions with regards to:
\begin{itemize}
    \item \textbf{Interest/Enjoyment:} Measured with four items from the Intrinsic Motivation Inventory (IMI) \cite{IMIhompage2023}, with scores averaged per IMI guidelines.
    \item \textbf{Comfort:} Assessed through seven self-designed questions to capture various aspects of comfort experienced during exoskeleton use.
    \item \textbf{Naturalness:} Evaluated with four self-designed questions about how participants perceived the movements of the exoskeleton, analyzed individually.
    \item \textbf{Passiveness:} Evaluated through four self-designed items to determine whether participants remained passive using the exoskeleton, with scores averaged to assess overall passiveness.
\end{itemize}

The full list of questions/items employed can be found in the \textit{Supplementary Materials}, Table VI. Participants filled in the questionnaires following a 7-point Likert scale, where, according to the question: (1) Very unnatural/uncomfortable/dissimilar - (7) Very natural/comfortable/similar or (1) Not true at all - (7) Very true. 

At the end of the experiment, participants also ranked---from (1) Favorite to (3) Least favorite---the three gait patterns in terms of overall experience, comfort, and naturalness. They also rated their confidence in these rankings, from (1) Not confident to (10) Very confident. Finally, we included open-ended questions (reported in the \textit{Supplementary Materials}) to capture additional insights and comments.

%\subsubsection{Sensors data}
Besides the participants' subjective experience, to determine whether walking along certain gait patterns led to increased human-robot interaction forces, the force measured by the original knee joint force sensor was recorded at a sampling frequency of \SI{100}{Hz} during the experiment. The \textbf{Mean Absolute Force} was then calculated per condition and leg, defined as the average magnitude of the force exerted at the right/left knee joints.


\subsubsection*{\textbf{Data analysis}}
\label{Sec:analysis}
    
We evaluated the effect of the different gait pattern conditions on the subjective and objective performance variables using a linear mixed model (LMM) of the form:
%
\begin{equation}
\label{eq:interaction}
Var = Pattern + Trial Order + (1|Participant),
\end{equation}
%
where $Var$ refers to any of the measured performance metrics (e.g., Comfort). The independent variable $Pattern$ refers to the pattern condition (i.e., \textit{Personalized}, \textit{Standard}, or \textit{Random}). The \textit{Standard} condition was chosen as the base condition, being equivalent for all the participants. To control for potential effects related to the sequence in which conditions were presented, we also included the $TrialOrder$ as an independent variable in the model. This ordinal variable represents the position of each pattern condition within the experimental sequence for each participant (i.e., \textit{First}, \textit{Second}, or \textit{Third}). We also included \textit{Participant} as a random factor. We fit the model using the \texttt{lmer} function from the \texttt{lme4} package in \texttt{R}.


Additionally, ranking outcomes were analyzed using a Friedman test, comparing across experimental conditions and trial order. After identifying significant differences with the Friedman test, a post-hoc Nemenyi test was conducted to explore pairwise comparisons between conditions. This analysis was performed using the \texttt{frdAllPairsNemenyiTest} function from the \texttt{PMCMRplus} package in \texttt{R}. We set all significance levels to $p<0.05$ and corrected for multiple comparisons with Bonferroni correction.


